Exploiting the Structure via Sketched Gradient Algorithms

Sketched gradient algorithms have been recently introduced for efficiently solving the large-scale constrained Least-squares regressions. In this paper we provide novel convergence analysis for the basic method {\it Gradient Projection Classical Sketch} (GPCS) to reveal the fast linear convergence rate of GPCS towards a vicinity of the solution thanks to the intrinsic low-dimensional geometric structure of the solution prompted by constraint set. Similar to our analysis we observe computational and sketch size trade-offs in numerical experiments. Hence we justify that the combination of gradient methods and the sketching technique is a way of designing efficient algorithms which can actively exploit the low-dimensional structure to accelerate computation in large scale data regression and signal processing applications.

==> GPIS_theory.tex <==

\section{Gradient Projection Iterative Sketch}
\label{sec:pagestyle}

Here we consider the combination of CS with the first order PGD algorithm the {\it Gradient Projection Classical Sketch} (GPCS):
\begin{equation} \label{eq:7}
    x_{i+1}=\mathcal{P}_\mathcal{K}(x_{i}-\eta (SA)^T(SAx_{i}-Sy)).
\end{equation}
Similarly we obtain the {\it Gradient Projection Iterative Hessian Sketch} (GPIHS) for solving IHS (\ref{eq:5}):
\begin{equation} \label{eq:8}
    x_{i+1}=\mathcal{P}_\mathcal{K}(x_i-\eta(A_s^TA_s(x_i-x^t)+mA^T(Ax^t-y)).
\end{equation}
Our proposed algorithm applies PGD to solve a sequence of sketched LS, starts with a CS step for a fast initialization, and then is followed by further iterations of IHS. We can observe from Algorithm \ref{A1} that sketches are constructed in the outer loop and within the inner loop we only need to access them. This property could be very useful when, for instance $A$ is stored in a slow speed memory and it is too large to be loaded at once into the fast memory. Also in large scale image reconstruction problems such as CT where due to its prohibited size $A$ is constructed on the fly.
 Note that thanks to the sketching each inner iteration of GPIS is $\frac{n}{m}$ times cheaper than a full PGD iterate in terms of matrix-vector multiplication, so intuitively we can see that there is potential in Algorithm 1 to get computational gain over the standard first order solver PGD. In the next section we provide the convergence analysis of GPIS and further discuss about this computational gain.





\begin{algorithm}[t]\label{A1}
\SetAlgoLined

 Initialization: $x_0^0 = 0$\;
 Given $A \in \mathcal{R}^{n \times d}$, sketch size $m \ll n$\;
 Prior knowledge: the true solution $x$ belongs to set $\mathcal{K}$ \;
  Generate a random sketching matrix $S^0 \in \mathcal{{R}}^{m \times n}$\;
  Calculate $S^0A$, $S^0y$\; 
 

 \While{$i=0:k_0-1$}{

       $x_{i+1}^0=\mathcal{P}_\mathcal{K}(x_{i}^0-\eta (S^0A)^T(S^0Ax_{i}^0-S^0y))$\;

       
 
 }
 $x_0^1 = x_{k_0}^0$\;
 \While{$t=1:N-1$}{
 Calculate $g=A^T(Ax_0^t-y)$\;
  Generate a random sketching matrix $S^t \in \mathcal{{R}}^{m \times n}$\;
  Calculate $A^t_s=S^tA$\; 
 

 \While{$i=0:k_t-1$}{

       $ x_{i+1}^t=\mathcal{P}_\mathcal{K}(x_i^t-\eta(A_s^{t^T}A_s^t(x_i^t-x_0^t)+mg))$\;

       
 
 }
 $x_0^{t+1}=x_{k}^t$\;

 }
 Return $x_{k}^N$\;
 \caption{Gradient Projection Iterative Sketch}
\end{algorithm}

\subsection{Convergence result}
%A theoretical analysis of the recursion behavior of GPIS is given in Theorem \ref{T1}. 
We start by defining certain properties of the operator $A$ and its interaction with the sketching scheme $S$, in a similar manner to the analysis in \cite{2015_Oymak_Sharp} and \cite{2015_Pilanci_Randomized}. %Throughout this part we denote by $\mathcal{C}$ be the smallest closed cone at $x^\star$ containing the set $\mathcal{K}-x^\star$.
\begin{definition}
Let $\mathcal{C}$ be the smallest closed cone at $x^\star$ containing the set $\mathcal{K}-x^\star$, 
%$\mathcal{S}^{d-1}$ be the unit sphere in $\mathcal{R}^d$,
$\mathcal{B}^{d}$ be the unit ball in $\mathcal{R}^d$, $z_1$ and $z_2$ be arbitrary fixed unit-norm vectors in $\mathcal{R}^n$. The contraction factor $\alpha(\eta,S^tA)$, the noise amplification factor $\beta(S^t,A)$, and the distortion factor $\gamma(S^t,A)$ are defined as:
\begin{align}
&\alpha(\eta,S^tA)=k_f\sup_{u,v \in \mathcal{C} \cap \mathcal{B}^d} (v^T(I-\eta A^TS^{t^T}S^tA)u),\\
&\beta(S^t,A)=k_f\sup_{v \in \mathcal{C} \cap \mathcal{B}^d} (v^TA^T\frac{S^{t^T}S^t}{m}z_1),\\
&\gamma(S^t,A)=k_f\sup_{v \in \mathcal{C} \cap \mathcal{B}^d} (v^T A^T( \frac{1}{m}S^{t^T}S^t-I)z_2),
\end{align}
  where, we set $k_f = 1$ if $\mathcal{K}$ is convex, and $k_f = 2$ if $\mathcal{K}$ is non-convex.
\end{definition}
 The contraction factor $\alpha(\eta,S^tA)$ determines the convergence speed of both GPCS and GPIHS, the noise amplification factor $\beta(S^t,A)$ determines the final accuracy, and the distortion factor $\gamma(S^t,A)$ determines the GPIHS's outer loop convergence speed. After defining these terms we are ready to state our convergence theorem for the GPIS algorithm for a general constrained set $\mathcal{K}$ and any randomized sketching operator $S^t$ satisfying (\ref{eq:5}):

\begin{theorem}\label{T1}
   (General convergence theory of GPIS) Starting from $x_0^0$, the following error bound holds:
   
   for $t = 0$ (the initialization loop by GPCS):
   \begin{equation}\label{eq:8}
        \|x_{i}^0-x^\star\|_2 \leq \alpha^i(\eta,S^tA)\|x_0^0-x^\star\|_2 +   \frac{m\eta\beta(S^t,A)}{1-\alpha(\eta,S^tA)}\|w\|_2,
   \end{equation}
   for $t \geq 1$ and $x^t_0:=x^{t-1}_{k_{t-1}}$  
   (the consecutive loops by GPIHS)
    \begin{equation}\label{eq:9}
    \begin{aligned}
       &\|x_{i}^t-x^\star\|_2 \leq \alpha^i(\eta,S^tA)\|x_0^t-x^\star\|_2  \\
       &+  \frac{m \eta}{1-\alpha(\eta,S^tA)}(\beta(\sqrt{m}I,A)\|w\|_2 + \gamma(S^t,A)\|x_0^t-x^\star\|_A).
    \end{aligned}
    \end{equation}
    %Note that the step $x^t_0:=x^{t-1}_{k_{t-1}}$ in Algorithm 1 links this recursive bound across the outer loop. 
\end{theorem}

\subsection{Results for Gaussian sketches and convex $\mathcal{K}$}

Theorem 1 provides us with a general framework to describe the convergence of GPIS in terms of the constants $\alpha$, $\beta$ and $\gamma$. In particular and for Gaussian sketches, these constants find explicit bounding expressions in terms of the sketch size $m$ and the complexity of the constraint cone $\mathcal{C}$. 
%We have expressions of these terms to the Gaussian Width of the set $\mathcal{W}(A\mathcal{C}\cap\mathcal{S}^{n-1})$ and the sketch dimension $m$ when we choose $S^t$ to be a Gaussian sketching matrix. 
For this, we use the Gaussian Width argument (see, e.g. \cite[Definition 3.1]{2012_Chandrasekaran_Convex}):

\begin{definition} \label{D2}
The Gaussian width $\mathcal{W}(\Omega)$ is a statistical measure of the size of a set $\Omega$:
\begin{align}
    \mathcal{W}(\Omega) = E_g\left( \sup_{v \in \Omega} v^Tg\right),
\end{align}
where $g \in \mathcal{R}^n$ is draw from i.i.d. normal distribution.
\end{definition}
The value of $\mathcal{W}(\mathcal{C}\cap\mathcal{S}^{d-1})$ is a very useful measurement of the tightness of the structure of $x^\star$, for example, if $x^\star$ is $s$-sparse and we model the sparsity constraint using an $l_1$ ball, we will have $\mathcal{W}(\mathcal{C}\cap\mathcal{S}^{d-1}) \leq \sqrt{2slog(\frac{d}{s}) + \frac{5}{4}s}$, which means the sparser $x^\star$ is, the smaller the $\mathcal{W}(\mathcal{C}\cap\mathcal{S}^{d-1})$ will be \cite[Proposition 3.10]{2012_Chandrasekaran_Convex}. As an illustration we now quantify the bounds in Theorem 1 in terms of the sketch size $m$ and the Gaussian width of the transformed cone  $\mathcal{W}:= \mathcal{W}(A\mathcal{C}\cap\mathcal{S}^{n-1})$.

\begin{corollary} \label{T1}
  Let $r_+(A)$ and $r_-(A)$ denote the maximum and minimum singular value of $A$, $b_m=\sqrt{2}\frac{\Gamma(\frac{m+1}{2})}{\Gamma(\frac{m}{2})}\approx\sqrt{m}$, $\theta$, $c$ and $c_1$ be small positive constants. Assume the constrained set $\mathcal{K}$ is convex and the entries of the sketching matrix $S$ is i.i.d drawn from Normal distribution. With step size  $\eta = \frac{1}{r_+^2(A)(b_m+2\mathcal{W}+ \theta)^2}$ and sketch size $m \geq (2\mathcal{W}+\theta)^2$, we can quantify the bounds in Theorem 1 as:
   \begin{equation}\label{eq:15}
   \begin{aligned}
        \|x_{i}^0-x^\star\|_2 &\leq (1-\frac{r_-^2(A)}{r_+^2(A)}\frac{(b_m-2\mathcal{W}- \theta)^2}{(b_m+2\mathcal{W}+ \theta)^2})^i\|x_0^0-x^\star\|_2 \\
         & + \frac{r_+(A)}{r_-^2(A)}\frac{m}{(b_m-2\mathcal{W}- \theta)^2}(1+ \frac{c}{\sqrt{m}})\|w\|_2, 
   \end{aligned}
   \end{equation}
   for $t \geq 1$ 
    \begin{equation}\label{eq:16}
    \begin{aligned}
       &\|x_{i}^t-x^\star\|_2 \leq (1-\frac{r_-^2(A)}{r_+^2(A)}\frac{(b_m-2\mathcal{W}- \theta)^2}{(b_m+2\mathcal{W}+ \theta)^2})^i\|x_0^t-x^\star\|_2 \\
       &+  \frac{r_+(A)}{r_-^2(A)}\frac{m}{(b_m-2\mathcal{W}- \theta)^2}(\|w\|_2+\frac{c}{\sqrt{m}}\|x_0^t-x^\star\|_A). 
    \end{aligned}
    \end{equation}
With probability at least $(1-e^{\frac{-\theta^2}{2}})(1-6e^{-c_1 c^2})$.
\end{corollary}
 The proof of Theorem 1 and Corollary 1 is omited here, but can be found in our technical report \cite{Tang2016Gradient}. From Theorem 1 we have demonstrated that the amplified noise-term $\beta(S^t,A)\|w\|_2$ determines the final accuracy of the GPCS loop, while the GPIHS loops' final accuracy is determined by $(\beta(\sqrt{m}I,A)\|w\|_2 + \gamma(S^t,A)\|x_0^t-x^\star\|_A)$. In Corollary 1 we have bounded these terms by:
 \begin{equation}
     \beta(S^t,A)\|w\|_2 \leq r_+(A)(\|w\|_2 + \frac{c}{\sqrt{m}}\|w\|_2),
 \end{equation}
 and,
 \begin{equation}
    \begin{aligned}
          &\beta(\sqrt{m}I,A)\|w\|_2 + \gamma(S^t,A)\|x_0^t-x^\star\|_A \\
          &\leq r_+(A)(\|w\|_2  + \frac{c}{\sqrt{m}}\|x_0^t-x^\star\|_A),   
    \end{aligned}
 \end{equation} 
Bounds (17) and (18) show that the GPCS loop has a noise amplification term $\frac{c}{\sqrt{m}}\|w\|_2$ which is inversely proportional to the squared root of the sketch size $m$, so the GPCS will converge at an accuracy level which is suboptimal due to the dimensional reductionreduction. However, GPCS give us fast convergence in the beginning. If we now continue with the GPIHS loops (after the GPCS) the term $\frac{c}{\sqrt{m}}\|w\|_2$ switches to $\frac{c}{\sqrt{m}}\|x_0^t-x^\star\|_A$, and $\lim \|x_0^t-x^\star\|_A \rightarrow 0$ for large enough number of outer loops $t$. Therefore this noise amplification due to the sketching is gradually eliminated.
 
 The proposed algorithm starts with a GPCS loop instead of GPIHS in order to avoid the computational cost of full gradient calculation demanded by GPIHS outer loop at the beginning. Of course the use of a Gaussian sketching matrix is not computationally efficient and in practice fast sketching techniques such as the FJLT \cite{2008_Ailon_Fast} \cite{2009_Ailon_Fast} or the random row subsampling\footnote{when the importance of the rows of $A$ are roughly the same, otherwise a sampling scheme with non-uniform probabilities need to be used.} should be used in order to significantly reduce or eliminate the cost of computing the sketch $SA$, detailed introduction of these fast sketching methods can be found in \cite[section 2.1]{2016_Pilanci_Iterative}.
 
 \subsection{Computational gain of GPIS through sketching}

Now we turn to the insights of the contraction factor $\alpha(\eta,S^tA)$ to understand the potential speed up can be achieved using GPIS. For comparison we mention a classical result on the convergence of the PGD (\ref{eq:3}) for solving the unsketched original problem (\ref{eq:2}) for a theoretically optimal step size $\eta = \frac{1}{r_+^2(A)}$:

   \begin{equation}\label{eq:17}
        \|x_{j}-x^\star\|_2 \leq (1-\frac{r_-^2(A)}{r_+^2(A)})^j\|x_0-x^\star\|_2
          + \frac{r_+(A)}{r_-^2(A)}\|w\|_2. 
   \end{equation}
   
If we assume the computational cost on the projection operator is negligible (just for the convenience of this part of the discussion), the computational cost of performing $j$ iterations of PGD is equal to computing $\frac{n}{m}j$ iterations of GPIS inner loop, we have the contraction factor for $j$ epochs of GPIS:

\begin{equation}
    \alpha^{\frac{n}{m}j} = (1-\frac{r_-^2(A)}{r_+^2(A)}\frac{(b_m-2\mathcal{W}- \theta)^2}{(b_m+2\mathcal{W}+ \theta)^2})^{\frac{n}{m}j}.
\end{equation}
   
If we compare $\alpha^{\frac{n}{m}}$ with the contraction factor $(1-\frac{r_-^2(A)}{r_+^2(A)})$ for PGD (associated with comparable computation), we can see that the convergence speed of each iteration of GPIS is penalized by the factor $\frac{(b_m-2\mathcal{W}- \theta)^2}{(b_m+2\mathcal{W}+ \theta)^2}$ but since each GPIS is $\frac{n}{m}$ times cheaper than a PGD iteration we can run more iterations to compensate this penalization. Hence there exists a sketch-size $m \geq (2\mathcal{W}+\theta)^2$ which can minimize $\alpha^{\frac{n}{m}j}$, whose precise value is a function of $r_+(A)$, $r_-(A)$,  and the Gaussian Width $\mathcal{W}(A\mathcal{C}\cap\mathcal{S}^{n-1})$. On the other hand we see that the larger $n$ is, the larger gain the GPIS can have over the PGD, we also observe this experimentally.



%When we compare the convergence expressions for GPIS and PGD in Corollary 1, the convergence speed of GPIS is depended on the factor $(1-\frac{r_-^2(A)}{r_+^2(A)}\frac{(b_m-2\mathcal{W}- \theta)^2}{(b_m+2\mathcal{W}+ \theta)^2})^i$ and meanwhile for the PGD is $(1-\frac{r_-^2(A)}{r_+^2(A)})^j$, and since each GPIS inner loop is $\frac{n}{m}$ times cheaper than PGD in terms of computation, we set $i=\frac{n}{m}j$ to equalize the computational cost for both. Then we describe the comparison of the progress of $j$ PGD iterations and $\frac{n}{m}j$ GPIS inner loop iterations by:

%\begin{equation}\label{eq:18}
%    f=\frac{1-(1 - \frac{r_-^2(A)}{r_+^2(A)}\frac{(b_m-2\mathcal{W}- \theta)^2}{(b_m+2\mathcal{W}+ \theta)^2})^{\frac{n}{m}j}}{1-(1 - \frac{r_-^2(A)}{r_+^2(A)})^j}
%\end{equation}


%We observe from (\ref{eq:18}) that when the condition number is near to 1, the PGD can converge faster than GPIS, but if the condition number is approximately beyond 10 which is slightly higher, the GPIS start to be much more advantageous.





==> conclusion.tex <==
\section{conclusion}

We proposed the GPIS algorithm for efficiently solving the constrained LS problem through marrying the merits of sketching meta-algorithms and projected gradient descent. We provide theoretical analysis to reveal its mechanism for computational efficiency. Finally we demonstrate the computational efficiency of GPIS algorithm over standard first order algorithms in solving large scale LS by numerical experiments.

==> experiment_v1.tex <==
\section{Experiments}
\subsection{Large data example}

We start our experiments on the GPIS algorithm by applying it to a toy example of constrained least squares in a large data setting  with $x^\star \in \mathcal{R}^{100}$ and is 10-sparse: (a) $A \in \mathcal{R}^{8192 \times 100}$; (b) $A \in \mathcal{R}^{1024 \times 100}$; the condition number of $A$ is set to be 100. The matrix $A$ in both cases are randomly drawn from a Normal distribution and then their singular values are linearly tuned up\footnote{just simply do SVD: $A=U\Sigma V^T$ and replace the diagonal of $\Sigma$ with \{1,2,...,100\}} in order to increase the condition number so that the system is not well-conditioned. (If the condition number is close to 1, the PGD converges very rapidly and there are no benefits in sketching.) We use the simplest sketching scheme which is random subselection and we chose the sketch size which is empirically good in the experiment, in (a) only $5\%$ of the rows are selected at each outer loop to construct the sketched LS; the inner loop number of GPIHS is set to be 20, which means the total number of multiplications within an outer loop is equal to one full gradient calculation (1 epoch); in (b) instead we chose $20 \%$ of the rows in each outer iterations and with the same principle we set the number of inner loops of GPIHS to be 5. In practice for a well or medium conditioned $A$, a good number of inner loop for GPIHS recursion should be $k_t \approx \frac{n}{m}$, for an ill-conditioned $A$ such as the CT operator used below, $k_t \approx \frac{2n}{m}$ appears to be a good choice. We also find  that it is good to choose the number of GPCS inner loops $k_0 = 2k_t$. We can see that as our theory has predicted, the GPCS can converge to a sub-optimal accuracy level with a small amount of computation. However if we wish to reach the same optimal accuracy as the PGD algorithm, we need to choose GPIHS or GPIS. The GPIS benefits from the warm start provided by the GPCS loop and is faster than GPIHS (we observe this more clearly in figure 1.a where a relatively larger scaled LS is constructed).  The GPIS can provide acceleration over the PGD with the most greedy step size.

 	\begin{figure}[H] \label{fig:2} %{\textwidth}
	\centering
		\includegraphics[width=7cm]{cls_plot_modi}
    \caption{{\footnotesize the illustration of the computational savings of GPCS, GPIHS and GPIS over the standard PGD solver on a $l_1$ constrained problem The $l_1$ norm projector is provided by SPGL1 toolbox \cite{van2007spgl1}}}
	\end{figure}
\subsection{fan beam CT reconstruction}

 In practice we don't usually have the exact knowledge about the exact constraints of $x^\star$, for example we might know an image is sparse in wavelet domain but not know how sparse ($l_0$ norm) it is, or what exactly is the image's TV-norm or $l_1$ norm of its wavelet coefficients, a popular solution in this scenario is to replace the projection onto the hard constraint by a proximal operator \cite{combettes2011proximal} to enforce the foreknown structure. In this subsection we test the performance of GPIS in solving the fan beam CT reconstruction problem, where the image is sparse in wavelet domain:

 \begin{equation}
     \hat{x} = \arg \min_x {\|Ax-y\|_2^2 + \lambda \|\Phi x\|_{1}},
 \end{equation}
 where the regularization factor $\lambda$ is set to be $2.5 \times 10^{-5}$ which is empirically good in this experiment. The fan beam CT operator $A$ is provided by AIR toolbox \cite{hansen2012air}, the $l_1$-norm proximal operator is provided by UnLocBox \cite{perraudin2014unlocbox}.
We set the measurement vector $y$ to be corrupted by Poisson noise and the $SNR \approx 35dB$ which typifies a medium dose energy, the size of the image to be 256 by 256, and the size of $A$ matrix to be $184320 \times 65526$. We compare the GPIS algorithm using a proximal operator, with the famous ISTA and FISTA \cite{2009_Beck_Fast} algorithm. For our proposed algorithm, in each outer loop, $10 \%$ of the rows of $A$ is randomly selected to construct the sketched LS, $k_t = 20$ for GPIHS loops(2 epochs, since the CT operator is highly ill-conditioned) and $k_0=40$ for GPCS loop. We find out that our proposed algorithm can be significantly faster than the ISTA and be slightly faster than FISTA with a fixed step-size, in terms of total flops count.
   	\begin{figure}[H] \label{fig:3} %{\textwidth}
	\centering
		\includegraphics[width=6cm]{ct_imamz}
	\caption{	{\footnotesize fan beam CT experimental results for the compared algorithms.}}
	\end{figure}
 	\begin{figure}[H] \label{fig:4} %{\textwidth}
	\centering
		\includegraphics[width=5cm]{ct_plotmz}
	\caption{	{\footnotesize fan beam CT experiment: error plot for the compared algorithms. Since FISTA is a momentum method, after it reaches the best accuracy it can get, it will slightly drift away as shown in the dot plot. Similar phenomenon is also mentioned and observed in \cite{o2015adaptive}. Hence we stabilize FISTA by replacing the iterations after it reaches the best accuracy by ISTA iterations.}}
	\end{figure} %\vspace{-1cm}


